Large-scale Deployment of Vision-based Tactile Sensors on Multi-fingered Grippers

Vision-based Tactile Sensors (VBTSs) show significant promise in that they can leverage image measurements to provide high-spatial-resolution human-like performance. However, current VBTS designs, typically confined to the fingertips of robotic grippers, prove somewhat inadequate, as many grasping and manipulation tasks require multiple contact points with the object. With an end goal of enabling large-scale, multi-surface tactile sensing via VBTSs, our research (i) develops a synchronized image acquisition system with minimal latency,(ii) proposes a modularized VBTS design for easy integration into finger phalanges, and (iii) devises a zero-shot calibration approach to improve data efficiency in the simultaneous calibration of multiple VBTSs. In validating the system within a miniature 3-fingered robotic gripper equipped with 7 VBTSs we demonstrate improved tactile perception performance by covering the contact surfaces of both gripper fingers and palm. Additionally, we show that our VBTS design can be seamlessly integrated into various end-effector morphologies significantly reducing the data requirements for calibration.

==> notused.tex <==
% To calibrate the proposed modular tactile sensor that may have variant dimensions, we propose a physics-based tactile sensor model and design a realistic tactile simulator to generate sensor outputs accurately and efficiently at scale for calibration. This eliminates the need for extensive data acquisition for each sensor. Since the cameras, lights, and elastomer materials are shared across all the sensors, the calibrated physics-based parameters can be reused across different sensors, resulting in significant calibration simplification for all the sensors on the GelGripper. 

% \subsection{Near-field Camera Model and Calibration}

% \textbf{Camera Geometry:}  The near-field camera geometry is modeled as perspective projection~\cite{hartley2003multiple} since the elastomer deformation is not negligible compared with its working distance. Specifically, a 3D surface point ${}^{\{C\}}\widetilde{\mathbf{X}}$ is projected to a 2D image point in the homogeneous coordinate ${}^{\{P\}}\mathbf{x}$:
% \begin{equation}
%     {}^{\{P\}}\mathbf{x} = \frac{1}{{}^{\{C\}}Z}
% 	\mathbf{K}
% 	{}^{\{C\}}\widetilde{\mathbf{X}},
% \end{equation}
% where $\{C\}$ and $\{P\}$ are the camera and the pixel coordinate frames, respectively, and $\mathbf{K}$ is the camera intrinsics. Assuming elastomer thickness is uniform and known, the camera geometry is calibrated before attaching the elastomer using~\cite{zhang2000flexible} to rectify lens distortions and obtain the intrinsics and extrinsics of the camera.

% \textbf{Camera Radiometry:} Since the perceptible region is located around the center of the camera's field of view, the vignetting effect is ignored, and the camera radiometry only models the photometric response. Color cameras are used and set with a fixed white balance gain, then each color channel has its own monotonic photometric response, $\{F_c\}_{c=R,G,B}$, that correlates image irradiance, $\{I_c\}_{c=R,G,B}$, to measured image intensity $\{M_c\}_{c=R,G,B}$ as $M_c=F_c(I_c)$. The photometric response is calibrated by estimating $\{G_c=F_c^{-1}\}_{c=R,G,B}$, where $G_c$ is a third order polynomial function~\cite{mitsunaga1999radiometric}. Then, the surface radiance, $\{L_c^{i,j}\}_{c=R,G,B}$, can be obtained from measured image intensity as $L_c^{i,j}=G_c\left(M_c^{i,j}\right)$, where $(i,j)$ is the pixel location.

% \subsection{Ground-truth Elastomer Surface Geometry Acquisition}
% An XYZ 3-axis linear trimming stage is utilized for ground-truth elastomer surface geometry acquisition as shown in \cref{fig:calibration}. The sensor is fixed at the bottom of the stage where the displacement in the X and Y directions can be adjusted. A 3D-printed cube probe is fixed by a mount with a flat base, perpendicular to the sensor contact plane. The stage coordinate frame $\{S\}$ is aligned with the flat base of the mount. The ${}^{\{S\}}Z=0$ is set by tuning the stage with the cube probe in the Z direction just before contact. The X and Y directions are set by adjusting the stage such that the cube probe appears near the center of the perceptible region of the sensor during contact. Having established $\{S\}$, the transformation from $\{S\}$ to $\{C\}$ can be calibrated by solving a perspective-n-point problem~\cite{lepetit2009ep}. The calibration performance is evaluated by the reprojection error.

% Having calibrated the XYZ stage, the cube probe can be replaced by any 3D-printed object. Using the visibility constraint for the calibrated camera, the depth map for the object can be obtained. The contact area then only preserves those pixels whose depth is within the range of the elastomer thickness. The contact-free area is filled with the depth map of the contact plane. Therefore, by mounting different objects with known geometry and physically adjusting the calibrated stage to any XYZ values, the resulting per-pixel elastomer surface geometry in the sensor can be computed as ground truth.

% \subsection{Near-field Lighting Model and Calibration}

% \textbf{Lighting Geometry:} The lighting geometry of the proposed compact tactile sensor is composed of multiple LEDs, and each one is assumed as a point source. Therefore, it is characterized by the light positions $\{{}^{\{C\}}\widetilde{\mathbf{S}}_k\}_{k\in[1, N]}$, where $N$ is the number of LEDs. Given the $k^{th}$ light position, the unit light direction pointing outwards from the surface $\bar{\mathbf{s}}_k$, and the light-surface distance $\|\mathbf{s}_k\|$ can be obtained. A 3D-printed calibration object that has two cylindrical sundials placed on the diagonal of a square mount is developed to estimate the light positions. The press of the calibration object onto the elastomer surface is carefully controlled using the calibrated XYZ stage such that the 3D geometry of the elastomer surface in $\{C\}$ is perfectly known. With each light turned on at a time, the camera shoots one image to estimate its light position. The shadow cue is adopted to derive the respective light directions for the two sundials using~\cite{sato2003illumination}. The light position is further determined using triangulation.

% \textbf{Lighting Radiometry:} Considering the relative energy spatial distribution emitted from the light and arrived at the surface, the lighting radiometry is determined by the radiation pattern of the light and the distance from the light to the surface point. The radiation patterns for the chosen LEDs are symmetrical. Thus, the lighting radiometry can be characterized by:
% \begin{equation}
%     \kappa_{k}^{i,j} = \eta_{k}\left(\left(-\bar{\mathbf{s}}_k^{i,j}\right)^\top\bar{\mathbf{p}}_k\right)^{\mu_k}/\|\mathbf{s}_k^{i,j}\|^2,
% \end{equation}
% where $\bar{\mathbf{p}}_k$ is the principle light direction pointing outwards from the $k^{\text{th}}$ light. $\eta_{k}$, $\mu_k$, $\bar{\mathbf{p}}_k$ are lighting radiometry parameters to be jointly calibrated with reflectance parameters.

% \textbf{Reflectance:}  Due to surface roughness, the actual appearance of the elastomer visualized from the camera
% is flatter than Lambertia, motivating the adoption of the physics-based generalized Lambertian model~\cite{nayar1995visual} to characterize the elastomer reflectance. Assume the elastomer is spatially uniform, the surface radiance illuminated under a particular light can be then modeled as:
% \begin{equation}
% \resizebox{0.91\linewidth}{!}{
% $\begin{cases}\label{eq:brdf}
%         L_c^{i,j}\left(\theta_{r}^{i,j}, \theta_{i}^{i,j}, \phi_{r}^{i,j}-\phi_{i}^{i,j};\rho_{c},\sigma\right) = \kappa^{i,j}\frac{\rho_c}{\pi}\max\left(0,\cos{\theta_i^{i,j}}\right)f_r^{i,j}\\
%         f_r^{i,j} = A + B\max\left(0,\cos{\left(\phi_r^{i,j}-\phi_i^{i,j}\right)}\right)\sin\alpha^{i,j}\tan\beta^{i,j}\\
%         A = 1.0 - 0.5\frac{\sigma^2}{\sigma^2+0.33}\\
%         B = 0.45\frac{\sigma^2}{\sigma^2+0.09}, 
%     \end{cases}$}
% \end{equation}
% where $\left(\theta_i^{i,j},\phi_i^{i,j}\right)$ and $\left(\theta_r^{i,j},\phi_r^{i,j}\right)$ are the light and viewer directions in a local coordinate frame with its $z$ axis aligned with the surface normal, and $\alpha^{i,j}=\max{\left(\theta_i^{i,j}, \theta_r^{i,j}\right)}$ and $\beta^{i,j}=\min{\left(\theta_i^{i,j}, \theta_r^{i,j}\right)}$. $\sigma$ and $\{\rho_c\}_{c=R,G,B}$ are respectively the surface roughness and albedo as reflectance parameters.

% To calibrate the lighting radiometry parameters for each light and the reflectance parameters of the elastomer surface, a 3D-printed sphere with a diameter of $3~mm$ is used as the calibration object. The sphere is pressed at $Q$ different locations using the calibrated XYZ stage onto the elastomer surface to a deformation height of its radius. At each press, the camera captures $N$ images, each with one LED lit at a time. Since the press is carefully controlled, the 3D surface geometry can be derived. With the calibrated light position, pixels in the shadow region can be known. Then, the calibration aims to solve a constrained nonlinear fitting problem:
% \begin{equation}
% \label{eq:calib_cost_fun}
% \resizebox{0.9\linewidth}{!}{
% $\begin{aligned}
%     &\min\limits_{\Gamma} \sum\limits_{q=1}^{Q}\sum\limits_{k=1}^{N}\sum\limits_{c=1}^3\sum\limits_{i=1}^H\sum\limits_{j=1}^W\left[G_c\left(M_{c,k, q}^{i,j*}\right) - \kappa_k^{i,j}\frac{\rho_c}{\pi}\cos\theta_i^{i,j}f_r^{i,j}\right]^2 
%     + \lambda\sum\limits_{k=1}^N\left(\eta_k - 1\right)^2   \\ 
%     &\mathrm{s.t.}\quad\quad i, j\in\mathcal{I}_k\cap\mathcal{S}, \|\mathbf{\bar{p}}_k\|=1, \mu_k\geq0, \sigma\geq0
% \end{aligned}$}
% \end{equation}
% where $\Gamma=[\eta_k,\mu_k,\mathbf{\bar{p}}_k,\sigma,\rho_c]$, $H$ and $W$ are the height and width of the image sensor in pixels, respectively. $\mathcal{I}_k$ is the non-shadow area of the $k^{th}$ image and $\mathcal{S}$ is the perceptible region of GelSight within the camera's field of view. $*$ means the measurement throughout the paper. 

% In (\cref{eq:calib_cost_fun}), the first term aims to minimize the square residuals of surface radiance, while the second term aims to encourage the light strength $\eta_k$ closer to $1$. Due to the high nonlinearity of the problem, it requires careful initialization. $\mathbf{\bar{p}}_k$ is initialized with its direction pointing towards the center of the perceptible region, conforming with the ideal sensor design. $\mu_k$ is initialized to $1.2$ estimated from the nominal radial attenuation pattern in the LED datasheet. $\eta_k$ and $\rho_c$ are all initialized to $1$, while $\sigma$ is initialized to $0.2$. With fair initialization, the optimization problem can be solved using the Levenburg-Marquardt algorithm. 

% The calibration performance is evaluated by the surface radiance error on a test image not seen during fitting. As is shown in \cref{fig:calibration} (B), the surface radiance error decreases with increasing number of presses for calibration. The error converges at $4$ presses, implying that with only $4N$ calibration images, the model parameters can be accurately and efficiently obtained. Since the proposed compact GelSight sensors share the same type of LEDs and elastomer material, the lighting radiometry and reflectance parameters can be calibrated only once. 

% Having these parameters, with all the LEDs simultaneously turned on at working condition, the overall surface radiance, $\widehat{L}_c^{i,j}$, follows the superposition principle and can be written as:
% \begin{equation}
%     \widehat{L}_c^{i,j}=\sum_{k=1}^NL_{c,k}^{i,j}.
% \end{equation}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth,trim=0cm 0cm 0cm 0cm, clip]{figures/placeholder.png}
%     \caption{\textbf{Simulator evulation}}
%     \label{fig:simulator}
% \end{figure}


% \begin{table}[tb!]
%     \caption{Tactile sensor evaluation under zero-shot calibration and individual calibration}
%     \centering
%     \label{tab:bom}
%     \resizebox{0.9\linewidth}{!}{%
%         \begin{tabular}{|c|c|c|}
%         % \toprule
%         \hline
%         \multirow{2}{*}{} & \multicolumn{3}{l}{Calibration} \\
%                   & method1   & method2  & method3  \\
%         error1            &           &          &          \\
%         error2            &           &          &         
%         \end{tabular}
% \end{table}




% \subsection{Sensor Simulator Evaluation}
% In addition to the factors introduced before, the cast shadow model~\cite{katz2007direct} and 
% the elastomer deformation model~\cite{si2022taxim} are also included in the tactile sensor simulator. Its performance is evaluated by the similarity between simulated outputs using ground-truth geometries and the real sensor outputs captured by the setup in \cref{fig:calibration}. 

% We 3D-print $20$ different objects in the tactile shape dataset~\cite{gomes2021generation} for capturing real sensor outputs. For each object, multiple real images (sensor outputs) are collected under different press locations and orientations. A total of $280$ real images are collected as the evaluation dataset. We use three metrics to compare the similarity between the real and the simulated sensor outputs: mean absolute error (L1), structural index similarity (SSIM), and peak signal-to-noise ratio (PSNR). The qualitative comparison between the real and simulated sensor outputs is shown in \cref{fig:simulator}. The quantitative similarity comparison using the mean and standard deviation of the three metrics on the evaluation dataset are summarized in \cref{tab:quant_gelsim}. As shown, the simulator is capable of producing highly accurate structural information (evaluated by SSIM) taking advantage of the proposed geometrical calibration method. The image intensity (evaluated by L1 and PSNR) is also well-simulated owing to the proposed lighting radiometry and reflectance calibration method. The simulated cast shadow regions are in strong agreement with the real ones, implying that the light positions can be well-calibrated using the proposed method.



% The EndoFlex sensor is composed of an endoskeleton encased in silicone with two embedded cameras for continuous sensing (Fig. 2). Each endoskeleton was designed to be one continuous piece with a pair of rigid segments and flexures to form joints. This design minimizes the number of parts required to fabricate one finger when compared to traditional rigid fingers. The flexure design was chosen for its high compliance and low deformation of individual elements to reduce silicone delamination. We 3D printed the endoskeleton using an Onyx One printer with Markforged Onyx plastic
% for its combination of high strength and relatively low tensile modulus when compared to other extruded plastics. This combination of properties allowed minimal force loss during actuation.

% A camera was mounted into each endoskeleton segment
% to prevent any shifting during actuation. Three sets of red,
% green, and blue LEDs were mounted with cyanoacrylate adhesive onto the rigid segment of the endoskeleton. They were
% spaced 90 degrees apart to create a colored light gradient
% for the GelSight algorithm. Finally, the endoskeleton was
% threaded with Piscifun Onyx Braided Fishing Line soaked in
% Smooth-On Universal Mold Release to reduce friction when
% cast in silicone. We chose to use cable-driven actuation to
% reduce potential camera-view obstructions and also so that
% we could more easily integrate the camera into the finger
% skeleton.
% A rigid three finger palm was designed with temporary
% fasteners to allow for fast replacement of damaged fingers
% or for future iterations. Fingers were positioned in a ‘Y’
% pattern with two fingers and an opposing thumb. The pair of
% fingers was spaced thirty degrees apart to distribute grasping
% force without creating collisions. The palm was designed to
% have a rounded feature with a polyurethane foam layer to
% add grasping ability. A separate rigid plate was designed to
% be fastened onto the Panda robotic arm. Three Dynamixel
% AX-12A servos were mounted between the plate and the
% palm and served as the actuation method for the fingers
% through double axle spools. The double axle design allowed
% for actuated contraction and extension of each finger. The
% palm, plate and spools were all printed with Markforged
% Onyx plastic using a Markforged Onyx printer.
% As part of our finger manufacturing process, which is
% fully shown in Fig. 3, a two part mold is designed for
% casting silicone to create the optically clear medium for
% the GelSight sensor. The mold was designed to hold the
% endoskeleton during the casting process which removed the
% need for fasteners or adhesives to hold the silicone layer. The
% mold had high curvature to create a rounded finger much
% like a human finger. One major benefit of the curved surface
% was the high reflection of lights within the silicone which
% aided in sensing by removing shadows of pressed objects.
% The mold design removed any air gap between the camera
% lens and cast silicone to minimize the refraction of light. The
% mold was produced using a Formlabs 2 SLA printer for its
% high resolution. To achieve the optical clarity required to use
% GelSight, the mold was incrementally sanded with sandpaper
% reaching 2000 grit.

% The modular fingers were then placed on our palm plate
% to create our completed gripper. We also note that this
% configuration can be changed to enable different types of
% grasps, although we chose an enveloping grasp to maximize
% the amount of sensing the gripper could obtain from grasping
% an object in its palm.


% The GelHand is assembled by 17 compact GelSight sensors in 6 different configurations and achieves a physical dimension similar to that of a human hand; see \cref{fig:gripper} for a schematic illustration of the structure of the GelHand. Specifically, the index, middle, ring, and litter fingers share the same design. Each finger consists of three serial revolute joints from the base located on the palm to the distal end, \ie the \ac{mcp}, \ac{pip}, and \ac{dip} joints, with a range between 0 and 90 degrees. Their physical connection is an aluminum shaft supported by two deep groove ball bearings and is fixed by screws and bushings. A pair of torsion springs are also introduced to the joint to maintain a 0 initial joint angle when subjected to no load. \cref{fig:gripper} shows the design details of a finger. The design of the thumb is similar to that of a finger (see in \cref{fig:gripper}). Furthermore, as a fully opposable thumb is considered to be a unique advantage of Homo sapiens for better throwing and clubbing~\cite{young2003evolution} and critical for human evolution~\cite{karakostis2021biomechanics}, one dedicated DoF is introduced to the carpometacarpal joint of the thumb with a 90-degree range of motion and is in a 45-degree-offset with respect to its \ac{pip} joint axis.   

% All the fingers and the thumb are connected to a human-like palm base. For easy assembly, the palm is divided into two parts, each of which is embedded in a compact GelSight sensor. Of note, the upper part of the palm as shown in \cref{fig:gripper} has a large region to be sensed; thus, two cameras are adopted in one GelSight sensor, showing the scalability of our design.

% To actuate the finger to realize human-like flexion and extension motions, one cable is routed at two sides of the finger phalanxes whose ends are merged in the palm base and three pairs of torsion springs are deployed as shown in \cref{fig:gripper}. When the cable is released, the tension in the cable vanishes, and the finger will be recovered to the initial position under the effect of the torsion spring. Then, the extension motion of the finger is realized. Each finger is designed as a cable-driven mechanism actuated by a dynamixel XC330X-T288-T servo motor for flexion and extension motions. During experimentation, we mount the GelHand to a 7-DoF Kinova Gen3 manipulator.

==> review.tex <==

1 	13869 	Summary:
In this paper, the author presents the design of a
vision-based tactile sensor (VBTS). The sensor is endowed
with low latency, easy integration, and effective
calibration. Individual sensor components are assembled
into grippers with different configurations and perform
basic grasping and manipulation tasks based on the tactile
feedback. The paper is written in good language with
illustrations of the contents and figures. Experiments are
completed with solid results to well prove the statements
and contributions of the work.

Questions and Problems:
1.	Section II - A. Theoretical Performance: As each
sensor board powers the MUC, camera, and LEDs, will the
power density being too high to avoid overheating of the
chips? Does the signal transmission delay change as the
working duration increases?

2.	Section II - A. Theoretical Performance: “a
standard frame size of S = 20 KB”. 
The author mentioned camera has a 2-megapixel image, yet it
seems unclear to compress this image down to 20KB. What
resolution is used for capturing the frame? 

3.	Section III: For calibration, what does the
training set look like? For GelSight, they use tinny metal
balls at different positions to obtain surface normal at
each x, y location with corresponding color intensity. What
instruments are used for calibration in this paper and how
the data is collected?

4.	Section III: How is “individual” calibration
carried out? What is the difference between the “zero-shot”
and “individual” calibration. From my understanding, the
“zero-shot" is trained on a reference sensor and conduct an
alignment process between the new sensor and the reference
sensor. And “individual” calibration just trains the model
by each sensor itself. 
If the key point of the zero-shot calibration is for model
transitioning across sensors, a comparison of error on new
sensors using old training set between “zero-shot” and
“individual” calibration is preferred.
 	 	

2 	13871 	
This work presents a fascinating integration of seven
vision-based tactile sensors (VBTSs) into a single hand
with 3 fingers and a palm. Additionally, the authors
develop a zero-shot way to calibrate their sensors and
synchronize multiple of them. The work is very intriguing
and novel from an integration standpoint. Overall, this
paper is well-written and defined, with nicely formulated
introduction and related works sections. Most of my
suggestions, which are listed below, are quite minor.

Related Work/Table 1
A lot of GelSight cameras in the previous years are
actually using CSI cameras instead of USB cameras. It is
true that the original GelSight did use USB, but now most
of them are using CSIs. This does mean that multiple
cameras can run at once, as long as you have the
corresponding number of Raspberry Pi’s. 

Real Deployment on GelGripper
“... with 110 degree ‘gaps’...” - make sure the first
quotation is facing the right way, it is a weird Latex
issue I believe
“To evaluate the performance of the proposed Gelgripper” -
remember to capitalize GelGripper

Fig. 5: I understand that the input raw captures are quite
dark, but is there any way for readers to see a brighter
image of the input captures? Just so that it is easier to
see what is happening. Again, understandable if that is
just not possible or worth it. This comment might also be
more relevant for Fig. 6.
Fig. 8: is there any way to provide a scale or a 3D depth
map so the reader can better understand the depth
characteristics?  

3 	13873 	
This paper introduces a large-scale multiple-fingered
system featuring a synchronized image acquisition scheme
and a modular sensor design. The synchronized image
acquisition scheme allows the gripper to capture tactile
images from various sensors with minimal delay, while the
modular design facilitates the fabrication and integration
of these sensors. Nevertheless, there are notable
limitations in the experimental evaluation of the proposed
zero-shot calibration method, as outlined below and
warranting serious consideration.

1. While the sensors are designed to be modular, it is
important to note that they may not “share the same
configuration” due to variations introduced during
fabrication and assembly. Therefore, the claim should be
revised to reflect this inherent variability.

2. Why use a learning-based calibration method as a
baseline? The zero-shot calibration should be compared to
the original mapping-based calibration method. Furthermore,
the authors should provide results from employing 50 images
for the baseline calibration method to verify the proposed
zero-shot method's superior data efficiency.
 	 	
